Planetary system LHS 1140 revisited with ESPRESSO and TESS

LHS 1140 is an M dwarf known to host two known transiting planets at orbital periods of 3.77 and 24.7 days. The external planet (LHS 1140 b) is a rocky super-Earth that is located in the middle of the habitable zone of this low-mass star, placing this system at the forefront of the habitable exoplanet exploration. We further characterize this system by improving the physical and orbital properties and search for additional planetary-mass components in the system, also exploring the possibility of co-orbitals. We collected 113 new radial velocity observations with ESPRESSO over a 1.5-year time span with an average photon-noise precision of 1.07 m/s. We determine new masses with a precision of 6% for LHS 1140 b ($6.48 \pm 0.46~M_{\oplus}$) and 9% for LHS 1140 c ($m_c=1.78 \pm 0.17~M_{\oplus}$), reducing by half the previously published uncertainties. Although both planets have Earth-like bulk compositions, the internal structure analysis suggests that LHS 1140 b might be iron-enriched. In both cases, the water content is compatible to a maximum fraction of 10-12% in mass, which is equivalent to a deep ocean layer of $779 \pm 650$ km for the habitable-zone planet LHS 1140 b. Our results also provide evidence for a new planet candidate in the system ($m_d= 4.8\pm1.1~M_{\oplus}$) on a ~78.9-day orbital period, which is detected through three independent methods. The analysis also allows us to discard other planets above 0.5 $M_{\oplus}$ for periods shorter than 10 days and above 2 $M_{\oplus}$ for periods up to one year. Finally, our analysis discards co-orbital planets of LHS 1140 b down to 1 $M_{\oplus}$. Indications for a possible co-orbital signal in LHS 1140 c are detected in both radial velocity and photometric data, however. The new characterization of the system make it a key target for atmospheric studies of rocky worlds at different stellar irradiations

==> Table_TTVresults.tex <==
\begin{table}[]
%\centering
\setlength{\extrarowheight}{3pt}
\caption{\label{tab:ttvs}Priors and posterior distributions for the radial velocity analysis (see Sect.~\ref{sec:rv3p}).}
\begin{tabular}{lcc}
 
 \hline 
{Transit \#} & $T_0$ (BJD) & TTV (min)  \\ 
\hline 
1 & $2458389.28715_{-0.00419}^{+0.00477}$ &  $-9.31_{-5.86}^{+6.72}$\\
2 & $2458393.07194_{-0.00403}^{+0.00364}$ &  $0.56_{-5.61}^{+5.05}$\\
3 & $2458396.85022_{-0.00231}^{+0.0023}$ &  $1.06_{-2.99}^{+3.0}$\\
4 & $2458400.62857_{-0.00234}^{+0.00236}$ &  $1.67_{-3.05}^{+3.09}$\\
5 & $2458404.40569_{-0.00264}^{+0.00277}$ &  $0.5_{-3.51}^{+3.73}$ \\
 \hline
 
 \end{tabular}

\end{table}
